Query Complexity of k-NN based Mode Estimation

Motivated by the mode estimation problem of an unknown multivariate probability density function, we study the problem of identifying the point with the minimum k-th nearest neighbor distance for a given dataset of n points. We study the case where the pairwise distances are apriori unknown, but we have access to an oracle which we can query to get noisy information about the distance between any pair of points. For two natural oracle models, we design a sequential learning algorithm, based on the idea of confidence intervals, which adaptively decides which queries to send to the oracle and is able to correctly solve the problem with high probability. We derive instance-dependent upper bounds on the query complexity of our proposed scheme and also demonstrate significant improvement over the performance of other baselines via extensive numerical evaluations.

==> latex_files/Correctness_Proof.tex <==
\section{Correctness of Algorithm \ref{algo:AdaptiveModeEstimation}}


==> original_citations.tex <==
@article{adaptiveKNN_original,
  author    = {Daniel LeJeune and
               Richard G. Baraniuk and
               Reinhard Heckel},
  title     = {Adaptive Estimation for Approximate k-Nearest-Neighbor Computations},
  journal   = {CoRR},
  volume    = {abs/1902.09465},
  year      = {2019},
  url       = {http://arxiv.org/abs/1902.09465},
  archivePrefix = {arXiv},
  eprint    = {1902.09465},
  timestamp = {Tue, 21 May 2019 18:03:36 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1902-09465.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{bestK_original,
  author    = {Haotian Jiang and
              Jian Li and
              Mingda Qiao},
  title     = {Practical Algorithms for Best-K Identification in Multi-Armed Bandits},
  journal   = {CoRR},
  volume    = {abs/1705.06894},
  year      = {2017},
  url       = {http://arxiv.org/abs/1705.06894},
  archivePrefix = {arXiv},
  eprint    = {1705.06894},
  timestamp = {Tue, 12 May 2020 17:15:19 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/JiangLQ17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
